Beyond Accuracy: Behavioral Dynamics of Agentic Multi-Hunk Repair

Automated program repair has traditionally focused on single-hunk defects, overlooking multi-hunk bugs that are prevalent in real-world systems. Repairing these bugs requires coordinated edits across multiple, disjoint code regions, posing substantially greater challenges. We present the first systematic study of LLM-driven coding agents (Claude Code, Codex, Gemini-cli, and Qwen Code) on this task. We evaluate these four state-of-the-art agents on 404 multi-hunk bugs from the PolyHunk dataset, yielding 1,616 repair trajectories for large-scale behavioral analysis. We employ fine-grained metrics to assess localization, repair accuracy, regression behavior, and operational dynamics across agents. We find that localization capability varies substantially, with Codex achieving the highest success rate (75.3%) and Qwen Code the lowest (40.4%). Repair accuracy also differs widely, ranging from 26.98% (Qwen Code) to 92.82% (Claude Code), and consistently declines with increasing bug dispersion and complexity (hunk divergence and spatial proximity). High-performing agents (Claude Code and Codex) demonstrate superior semantic consistency, achieving positive average regression reduction, whereas lower-performing agents often introduce new test failures. Notably, agents do not fail fast; failed repairs consume substantially more resources (33%-440% more input tokens) and require longer execution time (35%-330%). Additionally, we developed Maple to provide agents with repository-level context. Empirical results show that Maple improves repair accuracy of Gemini-cli by ~21% through enhanced localization. By analyzing fine-grained metrics and trajectory-level analysis, this study moves beyond accuracy to explain how coding agents localize, reason, and act during multi-hunk repair. Our findings underscore the impact of bug divergence and spatial proximity on multi-hunk repair success for coding agents.

==> proposed-approach.tex <==
\subsection{Structured Context Analysis}
\label{sec:approach}

Contemporary Large Language Models demonstrate remarkable capabilities in code understanding and generation. However, their effectiveness is fundamentally constrained by context window limitations when reasoning about large-scale software systems. While Retrieval-Augmented Generation (RAG) techniques address this limitation, they often rely on semantic embeddings that fail to capture the structural and syntactic relationships inherent in source code. Furthermore, existing approaches lack protocol-level standardization, hindering interoperability across LLM systems and toolchains.

We address these challenges through a structured code analysis system that provides LLMs with precise, context-aware access to Java codebases via the Model Context Protocol (MCP)~\cite{mcp-spec}. Our approach is guided by three principles: (1) code queries should leverage syntactic structure rather than treating source as unstructured text, (2) retrieved code should include only necessary context to minimize token consumption while maintaining semantic completeness, and (3) tools should communicate through standardized protocols to enable interoperability.

Formally, let $\mathcal{C} = \{f_1, \ldots, f_n\}$ denote a Java codebase with $n$ source files, where each file $f_i$ contains type declarations $\mathcal{T}_i$ and method declarations $\mathcal{M}_i$. A query $q = (q_t, s, c)$ consists of query type $q_t \in \{\textsc{class}, \textsc{method}, \textsc{code}\}$, search pattern $s$, and optional constraint set $c$. A result $r = (f, T, M, \ell_s, \ell_e, \text{code})$ contains source file $f \in \mathcal{C}$, containing type $T \in \mathcal{T} \cup \{\bot\}$ (where $\bot$ denotes undefined), containing method $M \in \mathcal{M} \cup \{\bot\}$, line range $\ell_s, \ell_e \in \mathbb{N}$, and extracted source text. The system returns a result set $\mathcal{R}(q, \mathcal{C})$ containing all matches with adaptive formatting to minimize token consumption.

\subsubsection{Index Construction}

The foundation of our approach is Abstract Syntax Tree analysis of Java source code. We build precomputed indices through lazy initialization where parsing and indexing occur on first tool invocation and persist throughout the session. This strategy enables immediate server startup while ensuring deterministic query response times once initialized. AST parsing provides precise identification of declaration start positions while eliminating false positives from comments or string literals, direct access to language constructs without manual pattern matching, and resilience to code formatting variations.

For each parsed AST, we extract type declarations with their names and source locations, and method declarations with their names and source locations. We build structural metadata maintaining mappings from type names to files, from types to their methods, and from line numbers to containing scopes. Since AST parsers provide node start positions but not explicit end positions for code blocks, we employ heuristic estimation to determine declaration end boundaries by examining subsequent member positions and file length.

Java parsing can fail due to syntax errors, incomplete code, or parser limitations. Our implementation employs a two-phase recovery strategy: first attempting standard parsing with full content, then removing package and import declarations (common sources of parser errors) and retrying if parsing fails. Files that fail both phases are logged but do not prevent indexing of remaining files, balancing completeness with correctness.

\subsubsection{Index Structure}

Efficient code retrieval requires precomputed indices enabling sub-linear query execution. We construct three complementary indices, each optimized for specific query patterns.

The type index $I_\mathcal{T}: \text{TypeName} \rightarrow \mathcal{P}(\text{File} \times \text{LineRange})$ maps type names to their declaration locations, where $\mathcal{P}$ denotes the power set since types may be declared in multiple files. This index supports \texttt{search\_class(T)} with direct lookup in $O(1)$ expected time and \texttt{search\_class\_in\_file(T, f)} with filtered lookup in $O(|I_\mathcal{T}(T)|)$ time.

Java allows multiple types with the same simple name in different packages. Rather than storing fully-qualified names, which would complicate queries, we store all declarations and present them with file paths during result presentation. This design prioritizes recall over precision, which is appropriate for LLM-assisted exploration where context helps disambiguate.

The hierarchical method index $I_\mathcal{M}: \text{TypeName} \rightarrow (\text{MethodName} \rightarrow \mathcal{P}(\text{File} \times \text{LineRange}))$ uses a two-level structure reflecting Java's scoping rules where methods are typically declared within types. This organization enables \texttt{search\_method\_in\_class(m, T)} with two-level lookup in $O(1)$ expected time while supporting method overloading. For global method searches without class constraints, \texttt{search\_method(m)} iterates over all types $T \in I_\mathcal{T}$ and aggregates results from $I_\mathcal{M}(T)(m)$, requiring $O(n_t)$ time where $n_t$ denotes the total number of types in the codebase.

The top-level method index $I_{\mathcal{M}_{\text{top}}}: \text{MethodName} \rightarrow \mathcal{P}(\text{File} \times \text{LineRange})$ maintains a flat mapping from method names to their locations. While Java does not support top-level methods, this index is maintained for language generality and remains empty for Java codebases.

Algorithm~\ref{alg:indexing} describes our index construction process. The algorithm processes files sequentially, extracts class-to-method mappings from AST parsing, and gracefully handles parse failures.

\begin{algorithm}[t]
\SetAlgoLined
\small{
\KwIn{Codebase $\mathcal{C}$}
\KwOut{Indices $I_\mathcal{T}, I_\mathcal{M}, I_{\mathcal{M}_{\text{top}}}$}
\ForEach{file $f \in \mathcal{C}$}{
    $\text{ast} \leftarrow \textsc{Parse}(f)$\;
    \If{$\text{ast} \neq \bot$}{
        Extract types $\mathcal{T}_f$ with line ranges\;
        Extract class-to-methods mapping $\phi_f: \mathcal{T}_f \rightarrow \text{Methods}$\;
        \ForEach{type $T \in \mathcal{T}_f$}{
            $I_\mathcal{T}(T) \leftarrow I_\mathcal{T}(T) \cup \{(f, \text{range}(T))\}$\;
            \ForEach{method $(m, \text{range}) \in \phi_f(T)$}{
                $I_\mathcal{M}(T)(m) \leftarrow I_\mathcal{M}(T)(m) \cup \{(f, \text{range})\}$\;
            }
        }
    }
    \Else{
        Log parse failure for $f$\;
    }
}
\Return{$I_\mathcal{T}, I_\mathcal{M}, I_{\mathcal{M}_{\text{top}}}$}\;
}
\caption{Index Construction}
\label{alg:indexing}
\end{algorithm}

Index construction has time complexity $O(n \cdot k)$ for parsing plus $O(n_m)$ for index updates, yielding $O(n \cdot k + n_m)$ overall, where $k$ denotes average file size in lines and $n_m$ denotes total method count. Space complexity is $O(n_t + n_m + n_{m,{\text{top}}})$ where $n_t$ denotes total type count and $n_{m,{\text{top}}}$ denotes top-level method count. For Java, $n_{m,{\text{top}}} = 0$, yielding $O(n_t + n_m)$ space dominated by methods since $n_m \gg n_t$.

\subsubsection{Query Processing}

Query processing proceeds in three phases: index lookup, code extraction, and result formatting.

For structured queries, lookup strategies vary by query type:

\begin{equation}
    \text{Lookup}(q) = \begin{cases}
        I_\mathcal{T}(s) & \text{search for class } s \\
        I_\mathcal{M}(T)(s) & \text{search for method } s \text{ in class } T \\
        \bigcup_{\text{all } T} I_\mathcal{M}(T)(s) & \text{search for method } s \text{ globally}
    \end{cases}
\end{equation}

Class queries perform direct lookup in $I_\mathcal{T}$ with $O(1)$ expected time. Class-scoped method queries perform two-level lookup in $I_\mathcal{M}$ with $O(1)$ expected time. Global method queries iterate over all types and aggregate results, requiring $O(n_t)$ time where $n_t$ denotes the total number of types.

For unstructured code snippet queries, we perform linear scanning with exact substring matching across all parsed files. While less efficient than indexed search, code snippet queries are inherently pattern-based and benefit from examining all potential matches across the codebase.

File-scoped queries support flexible file path matching through suffix comparison, allowing queries to specify either full paths or file name suffixes. This design accommodates common developer workflows where files may be referenced by simple names (e.g., \texttt{Main.java}) or relative paths (e.g., \texttt{src/main/Main.java}).

For each location $(f, \ell_s, \ell_e)$ returned by lookup, we extract source text with appropriate context. Class queries extract class signatures from declaration through opening brace, method queries extract method bodies from declaration to the estimated end position, and code queries extract the matched line plus $\delta$ lines of surrounding context where $\delta = 3$. The parameter $\delta$ balances providing sufficient context for understanding against minimizing token consumption.

To enrich results with scope information, we determine the containing type and method for each code location. Algorithm~\ref{alg:context} describes this process, which uses the hierarchical index to find the innermost containing scope.

\begin{algorithm}[t]
\SetAlgoLined
\small{
\KwIn{File $f$, line number $\ell$, indices $I_\mathcal{T}, I_\mathcal{M}$}
\KwOut{Containing type $T$, method $m$}
\ForEach{type $T$ in $I_\mathcal{M}$}{
    \ForEach{method $m$ in $I_\mathcal{M}(T)$}{
        \ForEach{$(f', [\ell_s, \ell_e]) \in I_\mathcal{M}(T)(m)$}{
            \If{$f' = f \land \ell_s \leq \ell \leq \ell_e$}{
                \Return{$T, m$}\;
            }
        }
    }
}
\ForEach{method $m$ in $I_{\mathcal{M}_{\text{top}}}$}{
    \ForEach{$(f', [\ell_s, \ell_e]) \in I_{\mathcal{M}_{\text{top}}}(m)$}{
        \If{$f' = f \land \ell_s \leq \ell \leq \ell_e$}{
            \Return{$\bot, m$}\;
        }
    }
}
\Return{$\bot, \bot$}\;
}
\caption{Context Determination}
\label{alg:context}
\end{algorithm}

Context determination requires $O(n_m)$ time in the worst case where $n_m$ denotes the total number of methods across all types, though early termination when a match is found typically yields better performance.

Each result is formatted using a custom tagging scheme that provides hierarchical context: \texttt{<file>}, \texttt{<class>}, \texttt{<method>}, and \texttt{<code>} tags delineate location metadata and source text.

When query results exceed threshold $\tau$, we apply adaptive summarization:

\begin{equation}
    \text{Format}(\mathcal{R}) = \begin{cases}
        \text{Full}(\mathcal{R}) & \text{if } |\mathcal{R}| \leq \tau \\
        \text{Full}(\mathcal{R}_{1:\tau}) \oplus \text{Summary}(\mathcal{R}_{\tau+1:}) & \text{if } |\mathcal{R}| > \tau
    \end{cases}
\end{equation}

where $\oplus$ denotes string concatenation, $\tau = 3$ is the result display threshold, and $\text{Summary}$ produces a condensed representation showing file paths and match counts without full code. This threshold balances token efficiency with information completeness.

\subsubsection{Tool Interface}

Our system exposes eight MCP tools organized by granularity and scope. Table~\ref{tab:tools} summarizes the tool suite.

% TODO: AST column and a checkbox
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Tool} & \textbf{Input} & \textbf{Returns} \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Global Scope}} \\
\quad\texttt{search\_class} & class name & Signature \\
\quad\texttt{search\_method} & method name & Body \\
\quad\texttt{search\_code} & code snippet & Match $\pm$3 \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Class Scope}} \\
\quad\texttt{search\_method\_in\_class} & method, class & Body \\
\midrule
\multicolumn{3}{@{}l}{\textbf{File Scope}} \\
\quad\texttt{search\_class\_in\_file} & class, file & Signature \\
\quad\texttt{search\_method\_in\_file} & method, file & Body \\
\quad\texttt{search\_code\_in\_file} & snippet, file & Match $\pm$3 \\
\quad\texttt{extract\_class\_skeleton} & file name & Signatures \\
\bottomrule
\end{tabular}
\caption{MCP tool suite organized by scope}
\label{tab:tools}
\end{table}

This design follows the principle of composability: complex queries can be constructed by chaining simpler tools. For example, understanding a class's implementation pattern requires extracting the class skeleton to see the API, searching methods in the class to examine specific implementations, and searching code patterns to find usage examples.

\subsubsection{MCP Integration}

Our system implements the Model Context Protocol specification, exposing code analysis capabilities as remotely-callable tools. We chose MCP over alternatives such as Language Server Protocol or custom REST APIs because MCP provides a standardized protocol for LLM-tool integration, its stdio-based transport eliminates network configuration complexity, and JSON Schema validation ensures type correctness at the protocol boundary.

We implement MCP through a framework approach~\cite{fastmcp} that handles low-level protocol mechanics while allowing high-level tool definition. The framework provides declarative tool registration, automatically generating JSON Schema specifications from function signatures and managing the complete JSON-RPC~\cite{jsonrpc-spec} communication layer.

The system uses the MCP STDIO transport~\cite{mcp-transport} where the client launches the server as a subprocess and establishes bidirectional communication through stdin/stdout pipes. Messages are UTF-8 encoded JSON-RPC structures delimited by newlines, with the protocol requirement that servers write only valid MCP messages to stdout while diagnostic information uses stderr. This framework handles message serialization, newline framing, JSON Schema validation of incoming requests, error propagation, and lifecycle management, allowing the implementation to focus on analysis logic rather than protocol compliance.

The STDIO transport eliminates network configuration, port management, and HTTP server infrastructure while providing process isolation and automatic resource cleanup. Sessions begin when the client spawns the server subprocess and persist through multiple message exchanges. The client sends \texttt{tools/list} requests for tool discovery and \texttt{tools/call} requests for invocations, with the server responding via JSON-RPC messages containing results or errors. This architecture enables natural integration with agentic workflows: the server process persists for the entire session, allowing the search index to initialize on first tool invocation and remain cached for subsequent queries.
While MCP supports asynchronous tool execution, our implementation uses synchronous processing, which simplifies the implementation while remaining sufficient for index-based query operations. The architecture supports future migration to async processing if needed.

Our design embodies three key principles. First, we optimize for recall over precision, ensuring LLMs receive all relevant results rather than risk missing critical information through aggressive filtering. Second, we provide general-purpose compositional primitives rather than domain-specific operations, maximizing applicability while enabling task-specific workflows through tool chaining. Third, we prioritize protocol standardization for interoperability over implementation-specific optimizations.
